Data-Driven Computational Imaging for Scientific Discovery

In computational imaging, hardware for signal sampling and software for object reconstruction are designed in tandem for improved capability. Examples of such systems include computed tomography (CT), magnetic resonance imaging (MRI), and superresolution microscopy. In contrast to more traditional cameras, in these devices, indirect measurements are taken and computational algorithms are used for reconstruction. This allows for advanced capabilities such as super-resolution or 3-dimensional imaging, pushing forward the frontier of scientific discovery. However, these techniques generally require a large number of measurements, causing low throughput, motion artifacts, and/or radiation damage, limiting applications. Data-driven approaches to reducing the number of measurements needed have been proposed, but they predominately require a ground truth or reference dataset, which may be impossible to collect. This work outlines a self-supervised approach and explores the future work that is necessary to make such a technique usable for real applications. Light-emitting diode (LED) array microscopy, a modality that allows visualization of transparent objects in two and three dimensions with high resolution and field-of-view, is used as an illustrative example. We release our code at https://github.com/vganapati/LED_PVAE and our experimental data at https://doi.org/10.6084/m9.figshare.21232088 .

==> scraps.tex <==
In particular, the aim is to develop methods that do not require a ground truth or reference dataset. 

hardware for signal sampling and software for object reconstruction are jointly designed for improved capability. In these systems,

Goal: reduce measurements, reduce reconstruction algorithm time, improve reconstruction quality

In computational imaging systems, hardware for signal sampling and software for object reconstruction are jointly designed for improved capability.  Examples include computed tomography (CT), magnetic resonance imaging (MRI), localization microscopy, and quantitative phase microscopy. In these systems, indirect measurements are taken, and computational algorithms are used for object reconstruction, allowing for advanced capabilities such as super-resolution or 3-dimensional imaging. Computational imaging systems generally require a large number of measurements, causing low throughput and motion artifacts. 

In computational imaging systems, indirect measurements are taken, and computational algorithms are used for object reconstruction

allowing for advanced capabilities such as super-resolution or 3-dimensional imaging. Computational imaging systems generally require a large number of measurements, causing low throughput, motion artifacts, and/or radiation damage. This program aims to reduce total measurement time by creating a self-supervised, data-driven, probabilistic framework.

Algorithm development with LED array microscopy will build the foundation for the PI’s research on other computational imaging methods such as micro-computed tomography and x-ray nano-holographic tomography.


A novel self-supervised, data-driven, probabilistic framework is proposed and validated 

This program aims to reduce total measurement time by creating a novel self-supervised, data-driven, probabilistic framework. 

Computational imaging aims to reconstruct some object, given noisy measurements. For high-quality reconstructions, a large number of measurements per object is generally needed, which may be costly or impossible to collect.

The proposed work improves the temporal resolution of light-emitting diode (LED) array microscopy, a modality that allows reconstruction of quantitative amplitude and phase (i.e., permittivity) in two and three dimensions with high resolution and high field-of-view. 


Measurements in computational imaging are taken with varying hardware parameters; in the case of LED array microscopy, the illumination pattern is varied to collect a stack of images. The proposed project will use simulated and experimental data to explore the impact of measurement parameter diversity over the object dataset for metrics of accuracy, stability, and robustness. A novel adaptive measurement technique, where the hardware parameters for object measurement are chosen based on the object data previously collected, will be prototyped and evaluated. Memory management techniques and considerations for video reconstruction will be created and assessed, with the significance of allowing developed frameworks to be applied to real experimental problems of high scientific interest.

The proposed algorithms will not require a ground truth or reference training dataset, unlike many other data-driven machine learning methods. 

The proposed work tackles the following problems that arise in finding the posterior: (1) construction of the prior $P(O)$ with no directly observed $O$, only measurements $M$ on each object of the set, (2) choice of the hardware parameters $p$ for every object $O$ to yield the correct $P(O)$, and (3) calculating $P(O | M)$ in a tractable manner. Our probabilistic formulation of the computational imaging problem permits uncertainty quantification, in contrast to most reconstruction algorithms that only yield a point estimate. Another key difference from standard methods is our joint reconstruction of a set of objects as opposed to consideration of a single object at a time. The use of information from multiple similar objects will allow for improved reconstructions with fewer measurements necessary per object.


To efficiently solve this problem, this program creates a novel technique through a reformulation of variational autoencoders. Crucially, no ground truth dataset is assumed, only noisy, sparse measurements on each object. 

, and LED illumination pattern in the case of LED array microscopy

Goal: reduce measurements, reduce reconstruction algorithm time, improve reconstruction quality



The CNN parameters are then co-optimized with the measurement matrix, using a ground truth dataset \cite{adler_deep_2016, Iliadis_DeepBinaryMask_2016, adler_block-based_2017, xie_adaptive_2017, mousavi_DeepCodec_2017, lohit_convolutional_2018, higham_deep_2018, du_fully_2017, grover_uncertainty_2019, qiao_deep_2020, bahadir_deep-learning-based_2020}. With this deep learning approach, sparsity in a known basis is not required, as all relationships are learned from the data. 

In computational imaging, hardware for data collection and software for post-processing are jointly designed. The ideas of compressed sensing may be directly applied to some computational imaging systems, such as the single pixel camera \cite{duarte_single-pixel_2008} and  magnetic resonance imaging (MRI) \cite{lustig_sparse_2007}. Other computational imaging systems may have physical constraints that do not permit a linear measurement matrix consisting of random projections. However, the idea of co-optimizing the measurement strategy with a CNN as the reconstruction algorithm can be applied to general computational imaging systems \cite{chakrabarti_learning_2016, robey_optimal_2018, haim_depth_2018, elmalem_learned_2018, diederich_using_2018, cheng_illumination_2019, cheng_deep_2019, muthumbi_learned_2019, hershko_multicolor_2019, hougne_learned_2020, Nehme_DeepSTORM3D_2020}. \ul{Since coming to Swarthmore College three years ago, I have established my group as a pioneer in using deep learning to jointly optimize the hardware and software in computational microscopy. In particular, my group was the first to demonstrate co-optimization of hardware and software parameters in an LED array microscope for object reconstruction} \cite{robey_optimal_2018}.


optimize the hyperparameters of the iterative reconstruction algorithm, some works also include the sampling strategy in the optimization \cite{sitzmann_end_2018}. Other works only optimize the sampling strategy, such as Refs. \cite{kellman_physics-based_2019, kellman_data-driven_2019}, where the illumination patterns in LED array microscopy are optimized in a data-driven fashion with an unrolled iterative solver.  In this case, the iterative solver has no trainable parameters, and thus may be less powerful in incorporating knowledge about the prior data distribution.

Deep learning has been demonstrated to be a powerful technique to reduce measurements with quality beyond what is available with compressed sensing. However, the necessity of a training dataset makes the technique prohibitive in many applications. A chicken-and-egg problem arises in the case of fragile or live specimens: without a reference object dataset, we cannot create a faster imaging method, but without the faster imaging method the training object dataset cannot be obtained. In the proposed work,

Our proposed work is also the first to take a comprehensive look at the problem. \ul{In particular, we propose to: (1) explore the impact of measurement pattern diversity on stability, robustness, and accuracy, (2) develop methods to work with large memory measurements and reconstructions, and (3) develop methods to account for temporal dependencies.}

STOPPED HERE

Why the variational autoencoder framework is useful
Outline the framework and describe the problem

Derivation of the Physics-Informed Variational Autoencoder

We aim to lower the number of measurements $n$ needed per object by utilizing information over the entire set of objects $\{O_1, O_2, ..., O_m\}$. 


How do we sense failure of joint optimization?
Can we detect rare events?
What are the applications?
Adaptivity
High-memory requirements of real applications, movies and for large scale FPM and real world CT

RESULTS: ALL FIGS FROM CAREER 2022 PROPOSAL
We hypothesize that if the measurement parameters $p$ are sufficiently diverse over the dataset (e.g.\ different illumination patterns for each object), high-quality reconstructions can be achieved with low $n$. 

The encoder and decoder in Fig.~\ref{fig:pvae} were in the form of a ``U-Net'' deep neural network architecture \cite{ronneberger_u-net_2015}, with the skip connections between the encoder and decoder parametrized as Gaussian distributions.

Tuning the $\alpha$ down causes sparser patterns to be more likely, and tuning all $\alpha \gg 1$ converges to a uniform brightness pattern. We propose to find what parameters $\alpha$ are optimal for given dataset attributes such as training dataset size, number of measurements per object, and signal-to-noise ratio of measurements.

Caption Notes:
Proposed Method: 1000 object dataset, 1 measurement each with multiplexed illumination

Standard Iterative Solution, 29 measurements with single LED illumination

Standard Iterative Solution, 1 measurement with multiplexed illumination



Results foam

dataset_foam_v2_pac1

noise_level_ind=1
num_examples_ind=1


\centering \caption{Phase reconstruction results ranked from highest to lowest peak signal-to-noise ratio (PSNR), from (a) ground truth, (b) physics-informed variational autoencoder (P-VAE) trained with 1,000 simulated measurements, (c) P-VAE with 100 simulated measurements, (d) iterative reconstruction with 29 single LED illuminated images, (e) P-VAE trained with 10 images, (f) P-VAE trained with 1 image.}


In many scenarios, the forward physics model is not completely known; there may be unspecified parameters. If the unspecified parameters vary for every measurement (e.g.\ partial coherence characteristics of a beam are time-dependent), they can be included as part of the object description $O$. If there are unspecified parameters that are constant throughout the entire dataset (e.g.\ pupil aberrations in LED array microscopy), they are included as trainable parameters in the function $P(M|O)$.

We aim to determine the effect of the distribution of measurement parameters $P(p)$ on reconstructions from the physics-informed variational autoencoder. Preliminary results demonstrate that measurement parameter diversity is important for improved reconstruction, see Fig.~\ref{fig:results_det}, where the peak signal-to-noise ratio (PSNR) is lower than in Fig.~\ref{fig:results_syn}, because $P(p)$ is deterministic (i.e.\ the same $p$ is used for every object $O$). 

We note that overtraining is a common problem when training a deep neural network to be a function approximator due to the large number of trainable parameters. We note that overtraining is not an issue in the outlined framework, as we aim to reconstruct \textit{only} the objects of the training dataset. 

Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.

\item Convergence tests
Does the framework, when hyperparameters are optimized with \textsc{hpo-uq}, achieve improved metrics for more objects $m$, more measurements $n$, and higher signal-to-noise ratios (i.e.\ pass convergence tests)?
More objects might need greater neural network capacity
Needs hyperparameter optimization

Show that higher SNR is actually worse, because it makes the framework unstable
More objects is worse, because the burden on the neural network is higher
more measurements is better

\item In what situations does the framework perform better than the state-of-the-art iterative solution, when both undergo hyperparameter optimization with \textsc{hpo-uq}? What is the increase in temporal resolution possible (e.g.\ for LED array microscopy, how many images need to be collected for the physics-informed variational autoencoder vs. an iterative solution to achieve a metric)?
\begin{enumerate}

\item Can poor reconstructions from the framework be predicted through the training loss when there is no ground truth or reference?

\item Can unusual or rare object examples in a dataset be accurately reconstructed with the framework?

\item Can we sense failure? correlation of loss metric to actual reconstruction loss of MSE, SSIM or PSNR

\item 
\end{enumerate}

The sensing of unusual or rare events is important for scientific applications. 

As the framework returns a posterior distribution that can be sampled, 
The probabilistic nature of the framework proposed here 
out of distribution error
Can poor reconstructions from the framework be predicted through the training loss when there is no ground truth or reference? correlation of loss metric to actual reconstruction loss of MSE, SSIM or PSNR

model mismatch for real data

In many scenarios, the forward physics model is not completely known; there may be unspecified or uncertain parameters. If the unspecified parameters vary for every measurement (e.g.\ partial coherence characteristics of a beam are time-dependent), they can be included as part of the object description $O$. If there are unspecified parameters that are constant throughout the entire dataset (e.g.\ pupil aberrations in LED array microscopy), they are included as trainable parameters in the function $P(M|O)$.

The impact of other hyperparameter choices including the architecture of the encoder and decoder networks, number of training iterations, and training rate will also be considered. We want results to be: (1) accurate, defined as average fidelity of samples of $P(O|M)$ to the true (synthetic) object by a metric such as mean-squared error, structural similarity, or peak signal-to-noise ratio, (2) robust, characterized by the worst-case loss (the negative of the right side of Eqn.~\ref{eqn:loss}) of multiple training runs with the same hyperparameters, and (3) stable, meaning small variance in loss among multiple training runs. 


approximately 2D specimen and 
 3D imaging more measurements are likely needed, see preliminary result in Fig.~\ref{fig:results_mnist} which shows visible improvement for $n=2$ over $n=1$. 

The goal is to achieve 3D object reconstruction with larger arrays of around 800 LEDs, as more LEDs in the illumination pattern generally mean higher resolution \cite{zheng_wide-field_2013}. For these large-scale, real-world problems, measurements required $\gg 1$. We note that results from this part can be applied in the future to computed tomography, where thousands of measurements are collected per object \cite{marchesini_sparse_2020, kuan_dense_2020}. 




A variational autoencoder traditionally uses deep neural networks to approximate the input-output functions of its encoder and decoder, a choice also taken for the physics-informed variational autoencoder in Part 1 of the proposed work. In Part 1, the measurements $M = [M_1, M_2, ..., M_n]$ on an object $O$ are the input to the encoder. These measurements must be processed by the encoder into a distribution $Q(z | M)$, which is done in a permutation invariant manner as described in Section~\ref{sec:arch}. The decoder samples $Q(z | M)$ and returns as output $P(O|z)$. To determine the training loss, the likelihood $P(M|O)=P(M_1, M_2, ..., M_n|O)$ must be computed, with the measurements being conditionally independent, $P(M_1, M_2, ..., M_n|O)\linebreak[1]=\linebreak[1]P(M_1|O) \linebreak[1] \times P(M_2|O) \times ... \times P(M_n|O)$. After training, reconstruction of all objects in the training dataset is possible. The current network architecture poses two problems: (1) if the number of measurements $n$ is large, backpropagation through the operation $P(M|O)$ and the encoder may be prohibitive in terms of memory, and (2) there is no procedure to reconstruct an object $O$ with measurements $M$ that is not included in the original training dataset. 

By assuming that the snapshots are independent (an assumption made with success in previous work by the PI's group using supervised learning \cite{cheng_deep_2019}), the previously discussed techniques can be applied directly. However, this frame-by-frame approach 

==> scraps2.tex <==

\begin{table}[h]
\centering
\begin{tabular}{| r | r |}
%Noise = 1e3
%Num Patterns = 1
%input_data = 'dataset_foam_v2_pac1'
%save_tag = 'foam_pac1'
%single pattern = False
%averaged over 10 examples

\hline
%P-VAE
\multicolumn{2}{|c|}{\textbf{P-VAE}}\\
\hline
   $m$ &   $n=1$\\
\hline
                  1          &            -4.71\\
                  10        &            -4.12\\
                  100      &             0.31\\
                  1,000   &            18.82\\
                  10,000 &            18.43\\
\hline
\hline
% Standard Iterative
\multicolumn{2}{|c|}{\textbf{Standard Iterative}}\\
\hline
   $n=29$ &   $n=1$ \\
\hline
   10.54 &  -3.96 \\

\hline
\end{tabular}

\caption{Comparison of peak signal-to-noise ratio (PSNR) values for the physics-informed autoencoder (P-VAE), varying the dataset size $m$; values are an average over 10 object examples. These values are compared with standard iterative methods.}
\label{table:foam_dataset_size_varypatt}
\end{table}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/results_synthetic.png}
\caption{Reconstruction results ranked from highest to lowest peak signal-to-noise ratio (PSNR). The result from the physics-informed variational autoencoder (P-VAE) is trained with a 1000 object dataset ($m=1000$), with 1 measurement per object ($n=1$). A comparison is given with standard iterative methods with a single LED illuminated in each measurement ($n=29$) and with a multiplexed illumination pattern ($n=1$).}
\label{fig:results_syn}
\end{figure}

%\begin{table}[h]
%\centering
%\begin{tabular}{| r | r |}
%%Noise = 1e3
%%Num Patterns = 1
%%input_data = 'dataset_foam_v2_pac1'
%%save_tag = 'foam_pac1'
%%single pattern = True
%%averaged over 10 examples
%
%\hline
%%P-VAE
%\multicolumn{2}{|c|}{\textbf{P-VAE}}\\
%\hline
%   $m$ &   $n=1$\\
%\hline
%                  1          &            -4.29\\
%                  10        &            -3.19\\
%                  100      &            -2.27\\
%                  1,000   &            2.13\\
%                  10,000 &            1.97\\
%\hline
%\hline
%% Standard Iterative
%\multicolumn{2}{|c|}{\textbf{Standard Iterative}}\\
%\hline
%   $n=29$ &   $n=1$ \\
%\hline
%   10.54 &  -4.39 \\
%
%\hline
%\end{tabular}
%
%\caption{Results with deterministic $P(p)$; comparison of peak signal-to-noise ratio (PSNR) values for the physics-informed autoencoder (P-VAE), varying the dataset size $m$; values are an average over 10 object examples. These values are compared with standard iterative methods.}
%\label{table:foam_dataset_size_fixedpatt}
%\end{table}





%\begin{figure}[h]
%\centering
%\includegraphics[width=0.375\textwidth]{figures/results_deterministic.png}
%\caption{A constant $p$ over the dataset results in reconstruction artifacts.}
%\label{fig:results_det}
%\end{figure}

\begin{wrapfigure}{l}{0.375\textwidth}
  \vspace{-3em}
  \begin{center}
    \includegraphics[width=0.375\textwidth]{figures/results_deterministic.png}
  \end{center}
  \caption{A constant $p$ over the dataset results in reconstruction artifacts.}
  \label{fig:results_det}
  \vspace{0em}
\end{wrapfigure}

%\begin{tabular}{rrrr}
%\hline
%   num\_patterns\_vec &   neural network &   all leds &   mult \\
%\hline
%                  1 &             7.55 &      21.17 &   0.07 \\
%                  2 &            14.47 &      21.17 &  -0.02 \\
%                  3 &            16.48 &      21.17 &   1.86 \\
%                  4 &            18.61 &      21.17 &   3.69 \\
%\hline
%\end{tabular}

The distribution of multiplexed illumination patterns $P(p)$ is a Dirichlet distribution as described in Section~\ref{sec:dataset}. We emulate measurements assuming a deterministic $P(p)$ (i.e.\ the same illumination pattern(s) $p$ is used for every object $O$), see Fig.~\ref{fig:dataset}. Results from training on this dataset demonstrate that measurement parameter diversity is important for improved reconstruction, see Fig.~\ref{fig:results_det}, where the peak signal-to-noise ratio (PSNR) is lower when $P(p)$ is deterministic.

We create a synthetic 3D MNIST dataset, consisting of two MNIST digits in axial planes $10$ $\mu$m apart. Each of the two MNIST digits is approximated as a thin phase object. 

Reconstruction with the stack of 29 single LEDs yields a PSNR of 21.17.

